Dealing with Uncertainty: The Value of Reputation in the Absence of Legal Institutions

This paper studies reputation in the online market for illegal drugs in which no legal institutions exist to alleviate uncertainty. Trade takes place on platforms that offer rating systems for sellers, thereby providing an observable measure of reputation. The analysis exploits the fact that one of the two dominant platforms unexpectedly disappeared. Re-entering sellers reset their rating. The results show that on average prices decreased by up to 9% and that a 1% increase in rating causes a price increase of 1%. Ratings and prices recover after about three months. We calculate that identified good types earn 1,650 USD more per week.

==> dn-model.tex <==
To illustrate the key elements of pricing by sellers in the market we analyse, we consider a simple, stylized model in the spirit of \citet{singh-vives-1984}. In line with our identification strategy, we abstract from the mechanics of reputation-building. Instead, we aim to understand the basic patterns of prices that result from the ratings system overcoming the uncertainty buyers face. 

Suppose there are two sellers indexed by $1$ and $2$ respectively that each produce a differentiated good. There is a continuum of consumers with a quasi-linear utility function, where the representative consumer maximizes his/her utility $U(q_1,q_2) = \alpha_1 q_1 + \alpha_2 q_2 -(q_1^2+2\gamma q_1 q_2 + q_2^2)/2$ subject to the prices of the two goods. Under certain conditions on the parameters $\alpha_i$ and $\gamma$, where $i=1,2$, the inverse demand function is given by $p_i = \alpha_i - q_i -\gamma q_j$, where $i\neq j$.\footnote{Specifically, we assume that $\alpha_i$ and $\gamma$ are positive, $1-\gamma^2>0$, and $\alpha_i -\alpha_j \gamma >0$. We further require quantities and prices to be positive.} Since sellers of illegal drugs are very likely to be capacity constrained, we assume that sellers in our model choose their quantity $q_i$, taking as given the choice of the competitor $q_j$. Then we find that in equilibrium, prices satisfy $p_i = (2\alpha_i - \gamma \alpha_j)/(4 + \gamma^2)$.\footnote{We ignore marginal cost for simplicity. As long as they are constant, this is without loss of generality, as prices can be considered to be net of marginal cost.}

Our stylized model allows us to capture two important aspects in a simple manner. One, the parameter $\alpha$ represents the given quality level of a seller. Setting $\alpha_1 \neq \alpha_2$ then captures a fixed quality difference among sellers. Two, the parameter $\gamma$ represents the extent of substitutability between products. Allowing for different degrees of substitutability is important, as we will show in \autoref{sec:Descriptives} that there exist large differences in the number of competing offers across drug types and regional markets and likely ease of finding close substitutes for buyers. 

The model makes the following straightforward predictions about what we should observe in a given product market. First, if buyers are unable to distinguish between sellers of different quality levels, $\alpha_1=\alpha_2$ in the demand function, and prices are chosen equally across quality levels. That is, the equilibrium consists of a pooling price. However, if buyers are able to distinguish between the qualities of sellers, the high-quality seller sets a higher price. This difference is increasing in the degree of quality differentiation. Hence there are returns to reputation if it reveals the type of the seller.  Second, the closer substitutes the two products are, the greater the effect of being able to distinguish different quality levels. That is, the `markup' in price that can be charged by revealing oneself as a good type in the market increases if offers by competing sellers are close substitutes. As it turns out, the sizes of our estimates will indeed show patterns that fit the predictions of our model.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "dn-draft"
%%% End:


==> dn-sensitivity.tex <==


In tables~\ref{tab:fs-nc} and~\ref{tab:iv-nc} in the appendix we repeat our main specifications when excluding the escrow covariate. The results are unaffected by exclusion of the variable.
\autoref{tab:ols} presents estimation results for a naive estimation approach of the effect of rating on price using OLS without the first-stage specification (\ref{first-stage-eqn}). We find a small, statistically significant effect of rating on price for Cannabis, but not for Cocaine, Amphetamine, or the full sample. This effect implies that a change in rating by one percent is associated with a change in the unit price by 0.12\%. These findings are broadly in line with previous literature on legal marketplaces that suggests that there are only small or no effects of rating on price \citep[e.g.][]{resnick2002,cabral2010,houser-wooders-06,cai2014}.

%% FIXME: This is both larger, and not in line with the current OLS. Either remove or cite somewhere else as complementary evidence.
% Our estimates in \autoref{tab:ols} are also in line with previous work on darknet marketplaces in \cite{espinosa-2018} who investigates a smaller platform and finds that a 10\% increase in positive evaluations is associated with 0.3-0.6\% higher prices.

Our main result in \autoref{tab:iv} demonstrates that these small effects are misleading, as we find a substantial price premium for having a higher reputation once we account for the endogeneity of rating via the forced re-entry of Evolution sellers. In addition, we find consistent, positive effects of escrow usage on prices that are statistically significant for the full sample and Cocaine and are similar in size to the ratings effect. The variation in effect size is in line with the differences in price level among the three different substances.

\input{tables/ols.tex}

\autoref{tab:pl} presents estimation results for a placebo exit in the period prior to the actual platform exit. We assume a placebo exit takes 11 weeks prior to the actual Evolution exit. We then consider an estimation window of 15 weeks prior to the placebo exit and 10 weeks after. This is equivalent to the estimation window we consider around the real exit. We find no statistically significant effects of rating on price, instead all of the estimates are very noisy. We find small, mostly positive effects of escrow usage on price that are equally statistically insignificant.

\input{tables/pl.tex}

\clearpage

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "dn-draft"
%%% End:


==> tables/fs-nc.tex <==
\begin{table}[h]
	\centering
	\captionsetup{width=\textwidth,justification=raggedright,singlelinecheck=off}
	\caption{The effect of re-entry on rating}
	%\small
	%\fontsize{14}{16}
	\begin{threeparttable}
		\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}} l*{5}{S[%
					table-number-alignment=center,
					table-figures-integer=2, table-figures-decimal=3,
					round-precision=3,
					table-space-text-pre={-},
					table-space-text-post={***}
					]}}
			\toprule
			\addlinespace[2em]
			& {All} & {Cannabis} & {Cocaine} & {Amphetamine} \\
			\midrule
			Re-entry x post           & -0.088{**} & -0.091  & -0.091  & -0.080  \\
									& (0.042)    & (0.065) & (0.074) & (0.079) \\
									& [0.035]	 & [0.161] & [0.221] & [0.310] \\
			\midrule
			Item-specific FE        & {\checkmark} & {\checkmark} & {\checkmark} & {\checkmark} \\	
			Time FE        			& {\checkmark} & {\checkmark} & {\checkmark} & {\checkmark} \\		
			Num. obs.               & {50254}	   & {27220}   & {14947}   & {8087}    \\
			%	R$^2$ (full model)      & 0.765       & 0.623   & 0.904   & 0.410   \\
			%	R$^2$ (proj model)      & 0.016       & 0.013   & 0.023   & 0.015   \\
			%	Adj. R$^2$ (full model) & 0.729       & 0.563   & 0.890   & 0.317   \\
			%	Adj. R$^2$ (proj model) & -0.135      & -0.142  & -0.115  & -0.141  \\
			Num. items\    			& {6656}        & {3708}    & {1854}    & {1094}    \\
			%	Num. groups: month2     & 6           & 6       & 6       & 6       \\
			\bottomrule
			%	\multicolumn{5}{l}{\tiny{More explanations here. $^{***}p<0.001$, $^{**}p<0.01$, $^*p<0.05$.}}
		\end{tabular*}
		\begin{tablenotes}[para,flushleft]\scriptsize
		  \item \textbf{Notes:} Results based on a linear model as specified in \autoref{sec:Approach} with weekly data. The sample is restricted to a time period around the evolution exit, from 15 weeks prior to 10 weeks after the exit. Standard errors clustered at seller-substance level given in parentheses, $p$-values in brackets. *, ** and *** denote p$<$0.1, p$<$0.05 and p$<$0.01, respectively.
		  % Item-specific fixed effects are seller $\times$ category $\times$ quantity.
		\end{tablenotes}
	\end{threeparttable}
	\label{tab:fs-nc}
\end{table}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../dn-draft"
%%% End:


==> tables/fs.tex <==
\begin{table}[h]
\centering
\captionsetup{width=\textwidth,justification=raggedright,singlelinecheck=off}
\caption{The effect of re-entry on rating}
%\small
%\fontsize{14}{16}
\begin{threeparttable}
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}} l*{5}{S[%
	table-number-alignment=center,
	table-figures-integer=2, table-figures-decimal=3,
	round-precision=3,
	table-space-text-pre={-},
	table-space-text-post={***}
			]}}
\toprule
\addlinespace[2em]
	& {All} & {Cannabis} & {Cocaine} & {Amphetamine} \\
	\midrule
	Re-entry x post         & -0.090{**} & -0.092  & -0.093  & -0.083  \\
							& (0.043) 	 & (0.065) & (0.076) & (0.082) \\
							& [0.035] 	 & [0.16]  & [0.22]  & [0.31] \\
	Escrow                  & 0.018{*}   & 0.018   & 0.021   & 0.011   \\
							& (0.011)    & (0.015) & (0.019) & (0.012) \\
							& [0.098]	 & [0.234] & [0.279] & [0.367] \\
	\midrule
	Item-specific FE        & {\checkmark} & {\checkmark} & {\checkmark} & {\checkmark} \\	
	Time FE        			& {\checkmark} & {\checkmark} & {\checkmark} & {\checkmark} \\		
	Num. obs.               & {50254}	   & {27220}   & {14947}   & {8087}    \\
%	R$^2$ (full model)      & 0.765       & 0.623   & 0.904   & 0.410   \\
%	R$^2$ (proj model)      & 0.016       & 0.013   & 0.023   & 0.015   \\
%	Adj. R$^2$ (full model) & 0.729       & 0.563   & 0.890   & 0.317   \\
%	Adj. R$^2$ (proj model) & -0.135      & -0.142  & -0.115  & -0.141  \\
	Num. items\    			& {6656}        & {3708}    & {1854}    & {1094}    \\
%	Num. groups: month2     & 6           & 6       & 6       & 6       \\
	\bottomrule
%	\multicolumn{5}{l}{\tiny{More explanations here. $^{***}p<0.001$, $^{**}p<0.01$, $^*p<0.05$.}}
\end{tabular*}
    \begin{tablenotes}[para,flushleft]\scriptsize
      \item \textbf{Notes:} Results based on a linear model as specified in \autoref{sec:Approach} with weekly data. The sample is restricted to a time period around the evolution exit, from 15 weeks prior to 10 weeks after the exit. Standard errors clustered at seller-substance level given in parentheses, $p$-values in brackets. *, ** and *** denote p$<$0.1, p$<$0.05 and p$<$0.01, respectively.
	  % Item-specific fixed effects are seller $\times$ category $\times$ quantity.
    \end{tablenotes}
  \end{threeparttable}
\label{tab:fs}
\end{table}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../dn-draft"
%%% End:


==> tables/iv-nc.tex <==
\begin{table}
	\centering
	\captionsetup{width=\textwidth,justification=raggedright,singlelinecheck=off}
	\caption{The effect of rating on price}
	%\small
	\begin{threeparttable}
		\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}} l*{5}{S[%
					table-number-alignment=center,
					table-figures-integer=2, table-figures-decimal=3,
					round-precision=3,
					table-space-text-pre={-},
					table-space-text-post={***}
					]}}
			\toprule
			\addlinespace[2em]
			& {All} & {Cannabis} & {Cocaine} & {Amphetamine} \\
			\midrule
			Rating (ihs)            & 0.763{*} & 0.455   & 0.273   & 1.882   \\
									& (0.434)   & (0.409) & (0.440) & (2.009) \\
									& [0.079]	& [0.266] & [0.536] & [0.349] \\
			\midrule
			Item-specific FE        & {\checkmark} & {\checkmark} & {\checkmark} & {\checkmark} \\	
			Time FE        			& {\checkmark} & {\checkmark} & {\checkmark} & {\checkmark} \\		
			Num. obs.               & {50254}     & {27220}   & {14947}   & {8087}    \\
			%	R$^2$ (full model)      & 0.992     & 0.963   & 0.965   & 0.967   \\
			%	R$^2$ (proj model)      & -0.303    & -0.098  & -0.065  & -1.902  \\
			%	Adj. R$^2$ (full model) & 0.991     & 0.957   & 0.961   & 0.962   \\
			%	Adj. R$^2$ (proj model) & -0.502    & -0.271  & -0.216  & -2.359  \\
			Num. items     & {6656}      & {3708}    & {1854}    & {1094}    \\
			%	Num. groups: month2     & 6         & 6       & 6       & 6       \\
			\bottomrule
			%	\multicolumn{5}{l}{\tiny{More explanations here. $^{***}p<0.001$, $^{**}p<0.01$, $^*p<0.05$.}}
		\end{tabular*}
		\begin{tablenotes}[para,flushleft]\scriptsize
		  \item \textbf{Notes:} Results based on a linear model as specified in \autoref{sec:Approach} with weekly data. The sample is restricted to a time period around the evolution exit, from 15 weeks prior to 10 weeks after the exit. Standard errors clustered at seller-substance level given in parentheses, $p$-values in brackets. *, ** and *** denote p$<$0.1, p$<$0.05 and p$<$0.01, respectively.
		  % Item-specific fixed effects are seller $\times$ category $\times$ quantity.
		\end{tablenotes}
	\end{threeparttable}
	\label{tab:iv-nc}
\end{table}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../dn-draft"
%%% End:


==> tables/iv.tex <==
\begin{table}
\centering
\captionsetup{width=\textwidth,justification=raggedright,singlelinecheck=off}
\caption{The effect of rating on price}
%\small
\begin{threeparttable}
	\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}} l*{5}{S[%
	table-number-alignment=center,
	table-figures-integer=2, table-figures-decimal=3,
	round-precision=3,
	table-space-text-pre={-},
	table-space-text-post={***}
	]}}
	\toprule
	\addlinespace[2em]
	 & {All} & {Cannabis} & {Cocaine} & {Amphetamine} \\
	\midrule
	Rating (ihs)            & 0.769{*} & 0.456    & 0.296   & 1.908   \\
							& (0.435)   & (0.410) & (0.448) & (2.025) \\
							& [0.077]	& [0.26]  & [0.51]  & [0.36] \\
	Escrow                  & 0.005     & 0.006   & 0.020   & 0.008   \\
							& (0.010)   & (0.013) & (0.014) & (0.027) \\
							& [0.644]	& [0.266] & [0.509] & [0.346] \\
	\midrule
	Item-specific FE        & {\checkmark} & {\checkmark} & {\checkmark} & {\checkmark} \\	
	Time FE        			& {\checkmark} & {\checkmark} & {\checkmark} & {\checkmark} \\		
	Num. obs.               & {50254}     & {27220}   & {14947}   & {8087}    \\
%	R$^2$ (full model)      & 0.992     & 0.963   & 0.965   & 0.967   \\
%	R$^2$ (proj model)      & -0.303    & -0.098  & -0.065  & -1.902  \\
%	Adj. R$^2$ (full model) & 0.991     & 0.957   & 0.961   & 0.962   \\
%	Adj. R$^2$ (proj model) & -0.502    & -0.271  & -0.216  & -2.359  \\
	Num. items     & {6656}      & {3708}    & {1854}    & {1094}    \\
%	Num. groups: month2     & 6         & 6       & 6       & 6       \\
	\bottomrule
		%	\multicolumn{5}{l}{\tiny{More explanations here. $^{***}p<0.001$, $^{**}p<0.01$, $^*p<0.05$.}}
	\end{tabular*}
	\begin{tablenotes}[para,flushleft]\scriptsize
	  \item \textbf{Notes:} Results based on a linear model as specified in \autoref{sec:Approach} with weekly data. The sample is restricted to a time period around the evolution exit, from 15 weeks prior to 10 weeks after the exit. Standard errors clustered at item-level given in parentheses, $p$-values in brackets. *, ** and *** denote p$<$0.1, p$<$0.05 and p$<$0.01, respectively.
	  % Item-specific fixed effects are seller $\times$ category $\times$ quantity.
	\end{tablenotes}
\end{threeparttable}
\label{tab:iv}
\end{table}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../dn-draft"
%%% End:


==> tables/ols-nc.tex <==
\begin{table}
	\centering
	\captionsetup{width=\textwidth,justification=raggedright,singlelinecheck=off}
	\caption{The effect of rating on price (OLS)}
	\small
	\begin{threeparttable}
		\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}} l*{5}{S[%
					table-number-alignment=center,
					table-figures-integer=2, table-figures-decimal=3,
					round-precision=3,
					table-space-text-pre={-},
					table-space-text-post={***}
					]}}
			\toprule
			\addlinespace[2em]
			& {All} & {Cannabis} & {Cocaine} & {Amphetamine} \\
			\midrule		
			Rating (ihs)            & -0.008  & 0.013{*} & -0.052  & -0.025  \\
									& (0.011) & (0.007)	 & (0.049) & (0.019) \\
									& [0.469] & [0.052]  & [0.292] & [0.189] \\
			\midrule
			Item-specific FE        & {\checkmark} & {\checkmark} & {\checkmark} & {\checkmark} \\	
			Time FE        			& {\checkmark} & {\checkmark} & {\checkmark} & {\checkmark} \\		
			Num. obs.               & {50254}     & {27220}     & {14947}      & {8087}    \\
%			R$^2$ (full model)      & 0.994   & 0.967     & 0.968   & 0.989   \\
%			R$^2$ (proj model)      & 0.000   & 0.000     & 0.002   & 0.000   \\
%			Adj. R$^2$ (full model) & 0.993   & 0.961     & 0.963   & 0.987   \\
%			Adj. R$^2$ (proj model) & -0.153  & -0.158    & -0.140  & -0.157  \\
			Num. gitem      & {6656}      & {3708}      & {1854}       & {1094}    \\
			%			Num. groups: month2     & 6         & 6         & 6          & 6       \\
			\bottomrule
			%	\multicolumn{5}{l}{\tiny{More explanations here. $^{***}p<0.001$, $^{**}p<0.01$, $^*p<0.05$.}}
		\end{tabular*}
		\begin{tablenotes}[para,flushleft]\scriptsize
		  \item \textbf{Notes:} Results based on a linear model as specified in \autoref{sec:Approach} with weekly data. The sample is restricted to a time period around the evolution exit, from 15 weeks prior to 10 weeks after the exit. Standard errors clustered at seller-substance level given in parentheses, $p$-values in brackets. *, ** and *** denote p$<$0.1, p$<$0.05 and p$<$0.01, respectively.
		  % Item-specific fixed effects are seller $\times$ category $\times$ quantity.
		\end{tablenotes}
	\end{threeparttable}
	\label{tab:ols-nc}
\end{table}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../dn-draft"
%%% End:


==> tables/ols-week-nc.tex <==
\begin{table}
	\centering
	\captionsetup{width=\textwidth,justification=raggedright,singlelinecheck=off}
	\caption{The effect of rating on price (OLS)}
	%\small
	\begin{threeparttable}
		\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}} l*{5}{S[%
					table-number-alignment=center,
					table-figures-integer=2, table-figures-decimal=3,
					round-precision=3,
					table-space-text-pre={-},
					table-space-text-post={***}
					]}}
			\toprule
			\addlinespace[2em]
			& {All} & {Cannabis} & {Cocaine} & {Amphetamine} \\
			\midrule		
			Rating (ihs)            & -0.005  & 0.014{**} & -0.048  & -0.009  \\
									& (0.010) & (0.006)    & (0.050) & (0.022) \\
									& [0.613] & [0.034]  & [0.337] & [0.671] \\
			\midrule
			Item-specific FE        & {\checkmark} & {\checkmark} & {\checkmark} & {\checkmark} \\	
			Time FE        			& {\checkmark} & {\checkmark} & {\checkmark} & {\checkmark} \\		
			Num. obs.               & {50254}     & {27220}     & {14947}      & {8087}    \\
%			R$^2$ (full model)      & 0.994   & 0.967     & 0.968   & 0.989   \\
%			R$^2$ (proj model)      & 0.000   & 0.000     & 0.002   & 0.000   \\
%			Adj. R$^2$ (full model) & 0.993   & 0.961     & 0.963   & 0.987   \\
%			Adj. R$^2$ (proj model) & -0.153  & -0.158    & -0.140  & -0.157  \\
			Num. gitem      & {6656}      & {3708}      & {1854}       & {1094}    \\
			%			Num. groups: month2     & 6         & 6         & 6          & 6       \\
			\bottomrule
			%	\multicolumn{5}{l}{\tiny{More explanations here. $^{***}p<0.001$, $^{**}p<0.01$, $^*p<0.05$.}}
		\end{tabular*}
		\begin{tablenotes}[para,flushleft]\scriptsize
		  \item \textbf{Notes:} Results based on a linear model as specified in \autoref{sec:Approach} with weekly data. The sample is restricted to a time period around the evolution exit, from 15 weeks prior to 10 weeks after the exit. Standard errors clustered at seller-substance level given in parentheses, $p$-values in brackets. *, ** and *** denote p$<$0.1, p$<$0.05 and p$<$0.01, respectively.
		  % Item-specific fixed effects are seller $\times$ category $\times$ quantity.
		\end{tablenotes}
	\end{threeparttable}
	\label{tab:ols-nc}
\end{table}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../dn-draft"
%%% End:


==> tables/ols.tex <==
\begin{table}
	\centering
	\captionsetup{width=\textwidth,justification=raggedright,singlelinecheck=off}
	\caption{The effect of rating on price (OLS)}
	%\small
	\begin{threeparttable}
		\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}} l*{5}{S[%
					table-number-alignment=center,
					table-figures-integer=2, table-figures-decimal=3,
					round-precision=3,
					table-space-text-pre={-},
					table-space-text-post={***}
					]}}
			\toprule
			\addlinespace[2em]
			& {All} & {Cannabis} & {Cocaine} & {Amphetamine} \\
			\midrule			
			Rating (ihs)            & -0.010    & 0.012{*}	& -0.057	& -0.025  \\
									& (0.011)   & (0.007)	& (0.049)	& (0.019) \\
									& [0.389]	& [0.066]	& [0.249]	& [0.190]	\\
			Escrow                  & 0.017{*}	& 0.013     & 0.027{**} & 0.007   \\
									& (0.009)   & (0.012)   & (0.012)	& (0.028) \\
									& [0.052]	& [0.264]	& [0.031]	& [0.801]	\\
			\midrule
			Item-specific FE        & {\checkmark} & {\checkmark} & {\checkmark} & {\checkmark} \\	
			Time FE        			& {\checkmark} & {\checkmark} & {\checkmark} & {\checkmark} \\		
			Num. obs.               & {50254}     & {27220}     & {14947}      & {8087}    \\
%			R$^2$ (full model)      & 0.994     & 0.967     & 0.968      & 0.989   \\
%			R$^2$ (proj model)      & 0.001     & 0.000     & 0.005      & 0.000   \\
%			Adj. R$^2$ (full model) & 0.993     & 0.961     & 0.963      & 0.987   \\
%			Adj. R$^2$ (proj model) & -0.152    & -0.157    & -0.136     & -0.157  \\
			Num. gitem      & {6656}      & {3708}      & {1854}       & {1094}    \\
%			Num. groups: month2     & 6         & 6         & 6          & 6       \\
			\bottomrule
			%	\multicolumn{5}{l}{\tiny{More explanations here. $^{***}p<0.001$, $^{**}p<0.01$, $^*p<0.05$.}}
		\end{tabular*}
		\begin{tablenotes}[para,flushleft]\scriptsize
		  \item \textbf{Notes:} Results based on a linear model as specified in \autoref{sec:Approach} with weekly data. The sample is restricted to a time period around the evolution exit, from 15 weeks prior to 10 weeks after the exit. Standard errors clustered at seller-substance level given in parentheses, $p$-values in brackets. *, ** and *** denote p$<$0.1, p$<$0.05 and p$<$0.01, respectively.
		  % Item-specific fixed effects are seller $\times$ category $\times$ quantity.
		\end{tablenotes}
	\end{threeparttable}
	\label{tab:ols}
\end{table}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../dn-draft"
%%% End:


==> tables/pl-nc.tex <==
\begin{table}
	\centering
	\captionsetup{width=\textwidth,justification=raggedright,singlelinecheck=off}
	\caption{The effect of rating on price with a placebo exit}
	\small
	\begin{threeparttable}
		\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}} l*{5}{S[%
					table-number-alignment=center,
					table-figures-integer=2, table-figures-decimal=3,
					round-precision=3,
					table-space-text-pre={-},
					table-space-text-post={***}
					]}}
			\toprule
			\addlinespace[2em]
			& {All} & {Cannabis} & {Cocaine} & {Amphetamine} \\
			\midrule		
			Rating (ihs)            & -9.263   & -1.946  & -14.133  & -796.339    \\
									& (11.817) & (8.861) & (35.826) & (33923.390) \\
									& [0.433]  & [0.826] & [0.693]  & [0.981]	\\
			\midrule
			Item-specific FE        & {\checkmark} & {\checkmark} & {\checkmark} & {\checkmark} \\	
			Time FE        			& {\checkmark} & {\checkmark} & {\checkmark} & {\checkmark} \\		
			Num. obs.               & {56487}    & {30661}    & {16076}    & {9750}      \\
			%			R$^2$ (full model)      & 0.959    & 0.939    & 0.403    & -0.550    \\
			%			R$^2$ (proj model)      & -4.071   & -0.133   & -19.053  & -105.204  \\
			%			Adj. R$^2$ (full model) & 0.954    & 0.931    & 0.322    & -0.740    \\
			%			Adj. R$^2$ (proj model) & -4.769   & -0.296   & -21.776  & -118.243  \\
			Num. items      & {6836}     & {3860}     & {1916}     & {1060}      \\
			%			Num. groups: month2     & 6        & 6        & 6        & 6         \\
			%	Num. groups: month2     & 6         & 6       & 6       & 6       \\
			\bottomrule
			%	\multicolumn{5}{l}{\tiny{More explanations here. $^{***}p<0.001$, $^{**}p<0.01$, $^*p<0.05$.}}
		\end{tabular*}
		\begin{tablenotes}[para,flushleft]\scriptsize
		  \item \textbf{Notes:} Results based on a linear model as specified in \autoref{sec:Approach} with weekly data. The sample is restricted to a time period that ends a week before the exit. We assume a placebo exit occurs 10 weeks prior and consider the 15 weeks leading up to the placebo exit and 10 weeks after. Standard errors clustered at seller-substance level given in parentheses. *, ** and *** denote p$<$0.1, p$<$0.05 and p$<$0.01, respectively.
		  % Item-specific fixed effects are seller $\times$ category $\times$ quantity. quantity.
		\end{tablenotes}
	\end{threeparttable}
	\label{tab:pl-nc}
\end{table}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../dn-draft"
%%% End:

